Attacking Black-box Recommendations via Copying Cross-domain User Profiles

Recently, recommender systems that aim to suggest personalized lists of items for users to interact with online have drawn a lot of attention. In fact, many of these state-of-the-art techniques have been deep learning based. Recent studies have shown that these deep learning models (in particular for recommendation systems) are vulnerable to attacks, such as data poisoning, which generates users to promote a selected set of items. However, more recently, defense strategies have been developed to detect these generated users with fake profiles. Thus, advanced injection attacks of creating more `realistic' user profiles to promote a set of items is still a key challenge in the domain of deep learning based recommender systems. In this work, we present our framework CopyAttack, which is a reinforcement learning based black-box attack method that harnesses real users from a source domain by copying their profiles into the target domain with the goal of promoting a subset of items. CopyAttack is constructed to both efficiently and effectively learn policy gradient networks that first select, and then further refine/craft, user profiles from the source domain to ultimately copy into the target domain. CopyAttack's goal is to maximize the hit ratio of the targeted items in the Top-$k$ recommendation list of the users in the target domain. We have conducted experiments on two real-world datasets and have empirically verified the effectiveness of our proposed framework and furthermore performed a thorough model analysis.

==> old_model.tex <==
\section{The Proposed Framework}
\label{sec:methodlogy}
In this section, we will first give an overview of the proposed framework, then provide further details for each of the frameworks components, and finally discuss how to learn the model parameters.


 %*************************************************************************************************************
\begin{figure*}[t]
\centering
{\includegraphics[width=0.945\linewidth]{{figures/framework_attack.pdf}}}
\caption{An overview of the proposed framework. It contains three major components: user profile selection in B domain, user profile crafting, and Injection Attack and queries.  \red{***users without target item*** Path }}\label{fig:framework}
%\vskip -0.14in
\end{figure*}
%*************************************************************************************************************

\subsection{An Overview of the Proposed Framework}

To perform attacking in recommender systems under black-box setting, we propose a reinforcement learning (RL) based attack method to learn the strategy of obtaining real user profiles by copying cross-domain user profiles.

The architecture of the proposed method is shown in Figure~\ref{fig:framework}. The model consists of three main components: user profile selection, user profile crafting, and injection attack and queries. 


The first component is to perform user profile selection for specific target item attack, which is proposed to select user profiles in source domain $B$. 
However, modeling this process of selecting with reinforcement learning technique is rather challenging  under limited resources (queries), since huge number of user profiles (discrete action space) in source domain $B$ might lead to inefficiency and ineffectiveness at the same time.  Moreover, not all the user profiles are useful to help attack the specific target item in target recommender systems. 
To address these challenge, we propose to adopt hierarchical-structure policy gradient~\cite{chen2019large,sutton1998introduction,williams1992simple} with masking mechanism to effectively and efficiently learn the strategy of selecting cross-domain user profiles, so as to maximize long-run rewards. 

% Most existing RL techniques cannot handle the large discrete action space problem as the time complexity of making a decision is linear to the size of action space~\cite{zhao2018recommendations,zhao2019deep,dulac2015deep,chen2019large}.


With the selected user profile from the first component, the second component is use profile crafting, which aims to further craft the user profile by considering the reduction of attack cost. 
The length of user profiles in cross-domain $B$ could be very diverse, and not all the interaction towards items in user profiles are helpful. Too long user profile might include some noise as well as increase the attacking budgets. Hence, we introduce the second step policy gradient network to craft the the user profiles by considering attacking cost issue. 


%In particular, we also introduce a policy gradient network  to design the length of user profile. 

The third component is to attack the target recommender system via copying cross-domain user profiles, as well as perform queries on the target recommender system to obtain some feedback (reward) for optimizing the whole framework. Next, we describe the details of each component in the proposed framework.


%More specifically, we construct a balanced hierarchical clustering tree over user profiles, where each leaf node is represent as a user profile and each non-leaf node is policy network. Selecting a user profile in this tree is to seek a path from the root to a certain leaf of tree.



%However, building reinforcement learning (RL) based attack method under black-box setting face challenges. 

%There are huge number of user profiles (action space in RL) in source domain B. Not all the user profiles are useful to help attack the specific target item in target recommender systems. Thus, the first challenge is how to reduce the searching space of action (user profiles) in reinforcement learning to effectively and efficiently select cross-domain user profiles for attacking the specific target items. 

%Moreover, the length of user profiles in cross-domain B could be very diverse. Not all the behaviours in user profiles are helpful. Too long user profile might include some noise as well as increase the attacking budgets. Hence, the second challenge is how to further craft the user profiles by considering attacking cost. 


%To address these challenges, the architecture of the proposed method is shown in Figure~\ref{fig:framework}. The model consists of three main components: user profile selection, user profile crafting, and injection attack and queries. 

%effectively attack the target recommender system under the black-box setting, we propose to a reinforcement learning (RL) based attack method to learn the strategy of obtaining real user profiles. 
%harness the power of policy gradient in reinforcement learning to deal with discrete action for attacking black-box recommendations, where the process of copying cross-domain user profiles can be regarded as a discrete Markov Decision Process (MDP).  The architecture of the proposed method is shown in Figure ~\ref{fig:framework}. The model consists of three main components: user profile selection, user profile crafting, and injection attack and queries.  

%The first component is to perform user profile selection for specific target item attack, which is proposed to choose user profiles in cross-domain system $B$. 
%However, modeling this process of selecting with reinforcement learning technique is rather challenging, since huge number of user profile (discrete action space) in cross-domain system $B$ might lead to in efficiency and ineffectiveness at the same time. Most existing RL techniques cannot handle the large discrete action space problem as the time complexity of making a decision is linear to the size of action space~\cite{zhao2018recommendations,zhao2019deep,dulac2015deep,chen2019large}.
%To address this challenge, we propose to adopt hierarchical-structure policy gradient~\cite{chen2019large,sutton1998introduction,williams1992simple} with masking mechanism to learn the strategy of selecting better user profile, so as to maximize long-run rewards. More specifically, we construct a balanced hierarchical clustering tree over user profiles, where each leaf node is represent as a user profile and each non-leaf node is policy network. Selecting a user profile in this tree is to seek a path from the root to a certain leaf of tree.





%To learn the strategy of selecting better user profile, we propose to harness the power of policy gradient in reinforcement learning to deal with discrete action for attacking black-box  recommendations.



\subsection{Attacking Environment}

The attacking black-box framework can be modeled as Markov Decision Process (MDP) $(S, A, P, R, \gamma)$. The definition of the MDP for reinforcement learning contains state space $S$, action set $A$, transition probability $P$, reward $R$, discount factor $\gamma$, defined as follows:


%We use an Markov Decision Process (MDP) to model the user profile selection process  . 

%We model the proposed evasion attack procedure as Markov Decision Process $(S, A, P, R, \gamma)$. The definition of the MDP contains state space $S$, action set $A$, transition probability $P$, reward $R$, discount factor $\gamma$.

 
\begin{itemize}
\item \textbf{State $S$.} A state $s_t$ at $t$ consists of all the intermediate injected user profiles at state $t$.

%The state $s_t$ at $t$ is represented by the tuple $(N^{B->A}_t, v^*)$, where $N^{B->A}_t$ contains a partial user profiles from $B$. \red{***what is the $s_1$***}


\item \textbf{Action $A$.} $A= \left \{ a_t =(a^u_t, a^l_t) \right \}$. The attacker is allowed to select user  $a^u_t=u^B_{i}$ from cross-domain system $B$ at state $t$, and then craft their length according to the action $a^l_t =\hat{T}^B_i$ before injecting into the target recommender system $Rec$. 

%So  a single action at time step $t$ is . However, simple performing actions in $B$ is too expensive, since the number of user profile  is too huge. \red{***clustering, related items.***}

\item \textbf{Transition probability $P$.} Transition probability $p(s_{t+1} |s_t, a_t)$ defines the probability of state transition from $s_t$ to $s_{t+1}$ when attack takes action $a_t$. %  We  assume that the MDP satisfies $p(s_{t+1} | s_t, a_t,..., s_1, a_1) =$

%Transition dynamics shows how the action $a_t$ changes the $Rec(\cdot, \cdot)$. 
 


\item \textbf{Reward $R$.}
The purpose of attacker is to attack target item $v^*$ in the target recommender system $Rec(\cdot, \cdot)$ with their desires (promotion/demotion). In this work, we focus on the promotion attack, where the target items can be recommended to users as many as possible. Note that the promotion attack process can be generalized to demotion attack.  Therefore, it is natural to define reward function on the basis of the Ranking evaluation measures.
We assign a positive reward for action $a_t$ when the target item $v^*$ belongs to the Top-$K$ recommended list for  specific users $u^*$. The reward function can be defined as Hit Ratio (HR@K), as follows:
\begin{align}
    r(s_t, a_t)
\left\{\begin{matrix}
1, & v^* \in y_{u^*,>k}, \\ 
0, & v^*  \notin  y_{u^*,>k}
\end{matrix}\right.
\end{align}
%Note that the promotion attack process can be transferred to demotion attack by modifying the reward functions. 
% we need to query the systems for some users $u^*$ to get the feedback from  $Rec(\cdot, \cdot)$. 

\item \textbf{Terminal.} The attacking process will stop when the number of actions reaches the budget $\triangle$. In addition, in the case when fewer user profiles is enough to successfully satisfies the promotion task, the process stop.

\end{itemize}


%contains the intermediate user profiles $N^{'}_t = \left \{  B^{'}_1, ..., B^{'}_t \right \}$ at time $t$, targeted item $v^*$, all the user profiles $1$ from other sources. $v^*$
    


%Note that user profile represents user's interacted behaviors such as clicked and purchased. 


    





 


\subsection{ User Profile Selection via Hierarchical-structure Policy Gradient}


%However, modeling this process of selecting with reinforcement learning technique is rather challenging, since huge number of user profile (discrete action space) in source domain $B$ might lead to inefficiency and ineffectiveness at the same time.  Moreover, not all the user profiles are useful to help attack the specific target item in target recommender systems. 


User profile selection aims to learn the strategy of selecting cross-domain user profiles. The challenges are how to handle large-scale discrete action space (user profiles) as well as achieve satisfied results under limited resources to interact with the target (black-box) recommender system.  Most existing RL techniques cannot handle the large discrete action space problem as the time complexity of making a decision is linear to the size of action space~\cite{zhao2018recommendations,zhao2019deep,dulac2015deep,chen2019large}. 
To address these challenge, we propose to utilize hierarchical-structure policy gradient network with marking mechanism to model the process of selecting user profile, as shown in the left part in Figure~\ref{fig:framework}.  More specifically, we construct a  hierarchical clustering tree over cross-domain user profiles, where each leaf node is represented as a user profile and each non-leaf node is policy network. Selecting a user profile in this  hierarchical clustering tree is to seek a path from the root to a certain leaf of tree.  



%At the same time, it is non-trivial to train the policy gradient networks to achieve satisfied results due to the limitations of interacting (querying) with the target recommender system by considering the budget issue in black-box attacking.

%Then, we introduce masking mechanism to further reduce the discrete action space according to the specific target item.  








\subsubsection{Hierarchical Clustering Tree over Cross-domain User Profiles}
$\\$

In the hierarchical clustering tree,  each leaf node is represented as a cross-domain user profile, while each non-leaf node is policy network.  To perform clustering over all cross-domain user profiles, we propose to employ the divisive approach to repeatedly divide each cluster (starting from whole user profiles) into smaller sub-clusters, such that leaf nodes under the same non-leaf node in hierarchical clustering tree might be more similar than leaf nodes under other non-leaf nodes. This hierarchical clustering over user profiles incorporates additional the similarity information of user profiles, where similar user profiles tend to be clustered into one subtree of the clustering tree. In other words, the similarity between user profiles under the same subtree tend to be large than user profiles under other subtrees. 



More specifically, we adopt the K-means clustering method based on user representations of cross-domain users.  Different features sources, such as user's attribute,  review comments, and the user-item interactions, could be used to represent users. In this paper, we adopt the user-item interactions $\mathbf{Y}^B$ to represent the users since the auxiliary information such as user's attribute and  review comments is not available. We use the user representations $\mathbf{p}^B \in \mathbb{R} ^{d}$ learned by matrix factorization (MF)~\cite{?} to measure similarity between users in the source domain $B$.  Note that the number of cluster centers is set to as the same number of child nodes in the hierarchical clustering tree, where we denote the number of child nodes as $c$. The relationship between depth of hierarchical clustering tree $d$, the number of leaf node $ |N^B|$, and the number of child  node $c$ can be defined as follows:

\begin{align}
  c^{d-1} < |N^B| = n^B \leqslant  c^d
\end{align}
and the number of non-leaf nodes of the tree is $\mathcal{I} =  \frac{c^d - 1}{ c-1}$.


%The action is to select user profiles from $B$. The user profiles involve the items user interacted with. It is necessary to consider all the item. However, directly performing one action requires searching in $O (n^B * m)$ space, which is too expensive, since the number of user  $n^B$ and items $m$ can be very huge. Therefore, we decompose the action into $a_t = (a_t^{(1)}, a_t^{(2)}, a_t^{(3)})$. First, $a_t^{(1)}$ is used to choose user profile $T^B_i$. Then, $a_t^{(2)}, a_t^{(3)}$ is proposed to select the starting position and ending position  $T^B_i$, such that can help save the budge of attacker.
%Therefore, we propose to encoder user profiles as a representation for reducing the action space to enable efficient exploration.

\subsubsection{Masking Mechanism}

$\\$

While cross-domain user profiles contain informative signal of items, not all the cross-domain user profiles are useful for attacking the specific target item with limited number of queries in target recommender systems. Only that user profiles related to the specific target items would be useful. Therefore, we need to tune the hierarchical clustering tree  with masking mechanism to
locate some percentage of related cross-domain user profiles for the target items. More specifically, for each target item,  we take an approach of masking the cross-domain user profiles which do not include the target item.  As shown in the left part in Figure~\ref{fig:framework},  the path from non-leaf node $3$ to node $7$ is masked, since the cross-domain profiles of user $u_7^B$ and $u_8^B$ do not include the target item (with pink color). As such, the cross-domain user profiles can not be explored by the RL agent, which might further help reduce the action space and locate helpful cross-domain user profiles to perform effective attack. 




\subsubsection{Hierarchical-structure Policy Gradient}
$\\$

With the hierarchical clustering tree, the purpose of user profile selection is to learn the policy $p(a_t^u|s^u_t)$ for seeking a path $a^u_t$ from the root to a certain leaf of tree at state $t$.   Each non-leaf node in the tree is a policy gradient network, which can be modeled as Multi-Layer Perceptron (MLP). As such, there are $\mathcal{I}$  policy gradient network with $\theta=\left \{ \theta_1, \theta_2,..., \theta_\mathcal{I}    \right \}$ in  the hierarchical clustering tree.




In particular, the policy networks at $node_i$ first takes the current state as input and outputs a probability distribution over all child nodes of $node_i$, and then chooses one child to move based on the probability.  And, the selection process keeps moving until reaching a leaf node (user profile), which can form the path as follows,
\begin{align}
   a^u_t=\left \{ a_{[t,1]}^u, a_{[t,2]}^u,..., a_{[t,d]}^u    \right \}
\end{align}
 

This selection process can be decomposed to multiple steps according to selected path $a^u_t$, as follows,

\begin{align}
    p^u(a_t^u|s^u_t) &=\prod^d p^u_d (a_t^u|\cdot, s^u_t) \\
 \nonumber   &=  p^u_{d} (a_{[t,d]}^u| s^u_t)  \cdot  p^u_{d-1} (a_{[t,d-1]}^u| s_t)  \cdots  p^u_{1} (a_{[t,1]}^u|s^u_t) 
\end{align}


We represent the state $s^u_t$ with target item $v^*$ and previous selected users $\mathcal{U}_t^{B \rightarrow A} = \left \{  u^B_1, ..., u^B_i, ..., u^B_{t} \right \}$. We combine them together with Multi-Layer Perceptron  (MLP).   To decide which path   is going to move, we estimate the probability distribution over  the child at $node_i$, as follows,


\begin{align}
    \mathbf{x}_{v^*} &= RNN(\mathcal{U}_t^{B \rightarrow A}),\\
    p^u_i(\cdot | s^u_t) &= softmax (MLP( [\mathbf{q}^B_{v^*}  \oplus  \mathbf{x}_{v^*}] | \theta_i^u))
\end{align}
where $\mathbf{q}^B_{v^*}  \in \mathbb{R} ^{d}$ is the pre-train item representation via Matrix Factorization (MF) in source domain $B$. We model the selected users $\mathcal{U}_t^{B \rightarrow A}$ at state $s_t$ with RNN model as the representation $\mathbf{x}_{v^*}$. $\oplus $ is concatenation operation.

An illustration example of the process of selecting cross-domain user profiles is shown in the left part in Figure~\ref{fig:framework}. We have 8 user profiles, and build a balanced hierarchical clustering tree with 3 depth over user profiles in source domain $B$. For given state $s_t$, the status point is initially located at the root ($node_1$), and moves to one of its child nodes to ($node_2$) according to the probability distribution given by the policy network \emph{PN-1} corresponding to the root ($node_1$). And the process of selecting can stop when  the state point arrives a leaf node in the tree, which is the user $u_3^B$'s profile. Note that at the state point $node_5$, the path from $node_5$ to leaf node $u_4^B$ is marked since the profile of source domain user $u_4^B$ does not include the currently attacking target item. The possible path for this selection is $a^u_t=\left \{ node_1, node_2, node_5, u_r^B \right \}$, as the path with  green color in Figure.










% \textbf{Step 1.} 

% encoder the user $u_i$ history profile $B(i)=\left \{ v_1, ..., v_j, ...  \right \}$ as embedding $\mathbf{x}_i$ learned by LSTM/Auto-Encoder:
% \begin{align}
%     \mathbf{x}_{i} = Encoder( \left \{ v_1, ..., v_j, ...  \right \})
% \end{align}

% \textbf{Step 2} select user profile 
% \begin{align}
%     p( \cdot | s_t) = softmax ( MLP (\mathbf{x}^* | \theta_u)) 
% \end{align}

% \textbf{Step 3} extract the key items from the selected user profile $u_i$ (for filtering some noise)
% \begin{align}
%     p(a_t | s_t) = Decoder (\mathbf{x}_i | \theta_v)) 
% \end{align}
% where $a_t = \left \{ v_1, ..., v_j, ..., v_l  \right \}$. Note that all the items in $a_t$  are from the  user $u_i$ history profile $B(i)$.







% \red{Questions}
% \begin{itemize}

%     \item  How to select a user profile (strategy)? Should we craft the selected user profile with decoder? 1) filter some missing items in RecSys A; 2) make filtering items?
%     \item How to guarantee the user profiles are real for $Rec$
%     \item budge = the number of queries + the length of fake user profile
%     \item reading comprehension [ starting node - ending node ], add some non-overlapping items in A
%     \item does it sample the same user profiles multi time?
% \end{itemize} 

 

% \red{Future Work }
% \begin{itemize}
%     \item To recommend blue/violent movies to children/students,  etc. collect the unhealthy items (blue/violent), define the children, bias (female/male, black/while)  by considering some specific group.
% \end{itemize} 



\subsection{User Profile Crafting}



%The selected cross-domain user profile includes the many overlapping items, where 

%With the selected cross-domain user profile for target items,

%User profile crafting aims to further craft the user profile by considering the reduction of attack cost. 

%After the user profile selection which is used to selecting specific user, we obtain its corresponding user profiles.

Not all the interaction towards items in cross-domain user profiles are helpful.
Directly injecting the raw user profiles into the target recommender system
may lead to increase the attacking budgets and include some noise.  To address this challenge, we propose a clipping operation to craft the raw user profiles via policy network, as shown in the middle of Figure~\ref{fig:framework}.

More specifically, we first discrete the length into 10 different levels as follows,
\begin{align}
W=\left \{ 10\%, 20\% , 30\% , 40\% , 50\% , 60\% , 70\% , 80\% , 90\% , 100\%   \right \}
\end{align}
Then, the policy network is introduced to to choose the action $a^l=w $ from $W$ from the set $W$ to decide the length we keep.  As the raw selected user profile includes the target item $v^*$,  the raw user profile is clipped around the target item with the window size $w$. As such, we can consider the forward and backward related items.  For example,  the selected raw profile of user $u_i^B$ with 10 items is as follows, 
\begin{align}
    P_{u_i}^B= \left \{ v_1\rightarrow   v_2\rightarrow   v_3\rightarrow   v_4\rightarrow    v^*_5\rightarrow   v_6\rightarrow   v_7\rightarrow   v_8\rightarrow   v_9\rightarrow   v_{10}  \right \}
\end{align}
If the policy network takes the action $a^l=50\%$, the new user profile through  the clipping operation can keep around $50\%$ raw user profile, as follows,
\begin{align}
    \hat{P}_{u_i}^B= \left \{ v_3\rightarrow v_4\rightarrow    v^*_5\rightarrow v_6\rightarrow v_7 \right \}
\end{align}


The state $s^l_t$ for model clipping operation can be decided by the selected user $u_i$ and target item $v^*$. We estimate the probability of choosing action $a^l$ over the set $W$ with the state $s_t^l$, as follows,

\begin{align}
    p^l(\cdot | s^l_t) &= softmax (MLP( [\mathbf{p}^B_{i}  \oplus  \mathbf{q}^B_{v^*}] |\theta ^l))
\end{align}
where $ \mathbf{p}_i \in \mathbb{R} ^{d}$  is the pre-train  user representation via MF in source domain.   


%\subsection{Policy Network}


% The objective of policy gradient  is to maximize the expected discounted cumulative rewards, as follows,

% where its approximate gradient  with respect to the parameters is as follows,
% \begin{align}
%      \triangledown_{\theta}  J(\pi _{\theta}) \approx  \mathbb{E}_{\pi_{\theta}} [  \triangledown_{\theta} \log \pi_{\theta}(a|s) Q^{\pi_\theta }(s,a)]
% \end{align}
% where $ \pi_{\theta}(a|s)$ means the probability of taking the action $a$ at the state $s$, and $Q^{\pi_\theta }(s,a)$ is the expected discounted cumulative rewards starting with $s$ and $a$, which can be estimated empirically by sampling trajectories following the policy $\pi_\theta$. 



\subsection{Injection attack and Queries}


To perform  attacking in black-box setting, we only have the query access to the target model and get query feedback consisting  of Top-$k$ recommended items for specific users. 


As shown in the right part of Figure~\ref{fig:framework},   the final real user profile $\hat{P}_{u_i}^B$  from source domain $B$ is first to copy into target model. Then, some users can make the queries with the target model and get some feedback for corresponding cross-domain user profile. If the target item  in  the recommended list, the attacker obtain positive reword for training.



==> old_problem.tex <==

% \subsection{Problem Statement}


% In a target recommender system  $A$ (denoted as $Rec(\cdot)$), we have a set of users $\mathcal{U}^A= \left \{ u_1^A, u_2^A, ..., u_{n^An }^A \right \}$ and a set of items $ \mathcal{V}^A = \left \{ v_1, v_2, ..., v_{m^A} \right \} $, where $n^A$ is the number of users and $m^A$ is the number of items. The user-item interaction matrix can be denoted as $\mathbf{Y}^A \in \mathbb{R} ^{n^A \times m^A} $, where an interaction $y^A_{ij}$ indicates that user $u^A_i$ interacted with item $v_j$ (e.g., clicked/bought), and 0 otherwise. In addition, we define user profile consisting of items he/she interacts in $\mathbf{Y}^A$. Specifically,  user $u^A_i$'s profile can be represented as follows:
% \begin{align}
%     P_{u_i}^A = \left \{ v_1 \rightarrow  ... \rightarrow  v_j \rightarrow  ... \rightarrow  v_l  \right \}
% \end{align}
% where   $ \rightarrow$ means sequence order .$l$ is the length of user profile and can differ from user to user.
% Let $N^A_u = \left \{  P_{u_1}^A, ..., T^A_{u_i}, ..., T^A_{{u_{n^A}}} \right \}$ denotes the set of profiles for all the users in target domain $A$. 

% We also define item profile as  $P_{v_j}$ which is the set of user who have interacted (purchased/clicked) with item $v_j$ in $\mathbf{Y}^A$ as follows:
% \begin{align}
%   P_{v_j}^A = \left \{ u^A_1\rightarrow   ...\rightarrow   u^A_i\rightarrow   ...\rightarrow   u^A_o  \right \}
% \end{align}
% where $o$ is the length of user and can differ from item to item. Let $M^A = \left \{   P_{v_1}, ..., P_{v_j}, ...,  P_{v_{m^A}} \right \} $ denote the set of item profiles in target domain $A$.



% In addition, the user-item interaction matrix  in source domain $B$ can be denoted as $\mathbf{Y}^B \in \mathbb{R} ^{n^B \times m^B} $, consisting of  user set $\mathcal{U}^B= \left \{ u_1^B, u_2^B, ..., u_{n^B}^B \right \}$ with the size $n^B$ and items set $ \mathcal{V}^B = \left \{ v_1, v_2, ..., v_{m^B} \right \} $ with the size  $m^B$. % , where $n^B$ is the number of users and $m^B$ is the number of items. Note that the items 



% The set of user profiles $N^B$  in source domain $B$ can be represented as follows:
% \begin{align}
%   N_u^B = \left \{  P_{u_1}^B, ..., P_{u_i}^B, ..., P_{u_{n^B}}^B \right \},\\
%     P_{u_i}^B= \left \{ v_1\rightarrow   ...\rightarrow   v_j \rightarrow   ...\rightarrow   v_l  \right \}
% \end{align}
% where $P_{u_i}^B$ represents user $u^B_i$ 's profile consisting of him/her interacting behaviours with items in cross-domain system $B$, and $n^B$ is the number of users in $B$.  Note that there are overlapping items  between target domain $A$ and source domain $B$, and $\mathcal{V}^B \subset  \mathcal{V}^A $. 



% The goal of target recommender system is to predict whether user $u^A_i$ likes the item $v_j$ as follows:
% \begin{align}
%     y^A_{ij} = Rec (P^A_{u_i}, P_{v_j}^A )
% \end{align}
% %\red{***Should we assume the RecSys performs prediction via inductive learning, where the embedding of users and items are learned via aggregation operation.***}

% Without generalization, we define the task of target recommender system is to predict a list of potential items for each user as top-$k$ ranking. We formally summarize this kind of recommendation as follows:
% \begin{align}
%     y^A_{i,>k} = Rec (P^A_{u_i}, M^A)
% \end{align}
% where $y^A_{i,>k} = \left \{ v_{[1]} , v_{[2]}, ..., v_{[k]} \right \}$ denotes as Top-$k$ candidate items for user $u^A_i$, and $k$ is the length of recommended items.
% Note that these  candidate items in $y^A_{i,>k}$ are ranked by $Rec(\cdot)$, where compared with item $v_{[i+1]}$, user $u^A_i$ is more likely to click/purchase item $v_{[i]}$.


% The scenario we want to specifically consider in this work is to build an attack $g(\cdot, \cdot)$, which mislead the target recommender system $Rec(\cdot)$ to promote target item $v^*$ via injecting user profiles from cross domain $B$, so that the target item $v^*$ can be involved into the $y^A_{i,>k} = \left \{ v_{[1]}, ..., v^*_{[j]} , ..., v_{[k]} \right \}$ for user $u^A_i$.% \red{(HR/NDCG)}. 


% To achieve this goal, we propose a black-box attacking framework for recommendations, in which once the model is well-trained, we keep it sealed and the attack has no access to its model structures, parameters, gradients, and training dataset. In our black-box setting, only query access to the target model is available and each query feedback consists of  Top-$k$ recommended items for pretend users (get reward). 





% %to inject some fake user profiles into the existing recommender system $Rec$ for affecting the prediction. Each fake user profile contains items, indicating  purchasing/clicking items' behaviors of users. 

% %However, generating fake user profiles is challenging since the user profiles should be real,  and can be avoided the %detection from the recommender system. In other words, the user profile should be as realistic as possible %\red{[unnoticeable]}, and imitate the behaviors of real user in the exiting recommender system.  To achieve this goal, we propose to copy the user profile from its enemy. 
% %For example, to attack the recommender system of Ebey, its enemies such as Amazon, Taobao and JD.com, can use their knowledge to sample some real user profiles and inject them into target Ebey $Rec(\cdot)$ for influencing the performance of recommender system. 



% %To attack the target recommender system $Rec (\cdot)$, 
% %the selected user profiles $N^{B->A} = \left \{  T^B_1, ..., T^B_i, ..., T^B_{H} \right \}$ are injected into $A$. The fake user can be represented as $ \left \{  u^B_1, ..., u^B_i, ..., u^B_{H} \right \}$ with the length $H$.

% % With fake user $\left \{  u^B_1, ..., u^B_i, ..., u^B_{H} \right \}$, the item profile can directly be affected as follows:
% % \begin{align}
% %     C^{'}_{j} = \left \{ u^A_1, ..., u^A_i, ..., u^A_o, ..., u^{B}_i, ....  \right \},\\
% %     M^{'} = \left \{  C^{'}_1, ..., C^{'}_j, ..., C^{'}_m \right \} 
% % \end{align}

% As generating fake user profiles easily detected by target recommender system, with the set of user profiles $N_{u}^B$ from cross-domain system $B$,  attacker $g(\cdot, \cdot)$ aims to select users from cross-domain system $B$ for target item ($v^*$), and then copy these user profiles into target recommender system,  as follows:
% \begin{align}
%     N_u^{B \rightarrow A} = \left \{  P_{u_1}^B, ..., P_{u_i}^B, ..., P_{H}^B \right \},\\
%     \mathcal{U}^{B \rightarrow A} = \left \{  u^B_1, ..., u^B_i, ..., u^B_{H} \right \}
% \end{align}
% where $\mathcal{U}^{B \rightarrow A}$ is the set of selected user by attacker with the size $H$ for specific target item, and $ P_{u_i}^B$ in user profiles set $N_u^{B \rightarrow A}$ is the user profile corresponding to user $u_i^B$.


% %profiles $N^{B->A} = \left \{  T^B_1, ..., T^B_i, ..., T^B_{H} \right \}$ and then inject into target recommender systems $A$.

% After injection attack in target domain $A$, the polluted user set ${\mathcal{U}^A}'$ and  the polluted  item profile $P_{v_j}^{'}$ in $A$ can be represented as follows;
% \begin{align}
% {\mathcal{U}^A}'= \left \{ u_1^A, u_2^A, ..., u_n^A, u_{n+1}^B,..., u_{n+H}^B  \right \}, \\
%     P_{v_j}^{'}= \left \{ u^A_1\rightarrow   ...\rightarrow   u^A_i\rightarrow   ...\rightarrow   u^A_o \rightarrow   ...\rightarrow   u^{B}_{n+1}\rightarrow   ....  \right \}, \\
%     {M^A}' = \left \{   P_{v_1}, ..., P_{v_j}^{'}, ...,  P_{v_{m^A}} \right \}
% \end{align}
% where $P_{v_j}^{'}$ denote as the profile of item $v_j$ polluted by the user $u_{n+1}^B$, and ${M^A}'$ is the set of  polluted item profiles.

% % $\mathcal{U}^A= \left \{ u_1^A, u_2^A, ..., u_n^A, u_{n+1}^B,..., u_{n+H}^B  \right \}$, and 

% % as follows:


% % \begin{align}
% %     C^{'}_{j} = \left \{ u^A_1, ..., u^A_i, ..., u^A_o, ..., u^{B}_i, ....  \right \},\\
% %     M^{'} = \left \{  C^{'}_1, ..., C^{'}_j, ..., C^{'}_m \right \} 
% % \end{align}
% % where the selected user profiles denoted as $N^{B->A} = \left \{  T^B_1, ..., T^B_i, ..., T^B_{H} \right \}$ are injected into target recommender system $A$. The fake user can be represented as $ \left \{  u^B_1, ..., u^B_i, ..., u^B_{H} \right \}$ with the length $H$.

% % $N^{B->A}$ and infect the item profiles $M^{'}$


% % Given , the attack $g(\cdot, \cdot)$ aims to select some 

 
% %Given a learned recommender system $Rec (\cdot)$ and the set of user profiles $ N^B$ from cross-domain system $B$,  attacker $g(\cdot, \cdot)$ aims to select some user profile $N^{B \rightarrow A}$ and infect them into target system $A$.

% For the target attacking item $v^*$,  the goal of attack $g(v^*)$ is to promote it to users as many as possible. Mathematically, it can be summarize as
% \begin{align}
%     max \sum _{i=0}^{n^A} \mathbf{1} (v^* \in y^A_{i,>k}) \\
% s.t., y^A_{i,>k} = Rec (P^A_{u_i}, {M^A}'), \\
% |N_u^{B\rightarrow A}| \leq \triangle, \\
% {M^A}' \leftarrow N_u^{B\rightarrow A}= g(v^*)
% \end{align} 
% The attacker has a certain budget of $\triangle$ for each targeted item $v^*$ to attack the prediction of recommendation, such that the targeted $v^*$ item is appear to the list of users as many as possible.

% %


